What Exactly is an Insight? A Literature Review

Insights are often considered the ideal outcome of visual analysis sessions. However, there is no single definition of what an insight is. Some scholars define insights as correlations, while others define them as hypotheses or aha moments. This lack of a clear definition can make it difficult to build visualization tools that effectively support insight discovery. In this paper, we contribute a comprehensive literature review that maps the landscape of existing insight definitions. We summarize key themes regarding how insight is defined, with the goal of helping readers identify which definitions of insight align closely with their research and tool development goals. Based on our review, we also suggest interesting research directions, such as synthesizing a unified formalism for insight and connecting theories of insight to other critical concepts in visualization research.

==> old/protest-example.tex <==



\section{Illustrative Example}
\label{sec:protest_example}

Throughout this section, we demonstrate how to use \model\ by recreating a data analysis scenario from Mathisen et al.~\cite{mathisen_insideinsights_2019}, which follows a fictional analyst, John, as he investigates crime peaks in Baltimore from 2012 through 2015. John's analysis uncovers the first crime peak on April 27, 2015 which coincides with protests sparked by the funeral of Freddie Gray, a young black man who was killed by the Baltimore police. An overview is provided in \autoref{fig:crimetask-overview}, where each node represents a particular \model{} object that we create throughout the example, and the edges between nodes represent relationships between objects.

%To develop domain knowledge, analysts extract information through database searches or field investigations~\cite{pirolli_sensemaking_2005,gotz_interactive_2006,mathisen_insideinsights_2019}. 

%Consider, for example, our fictional analyst, John, who is investigating crime peaks in Baltimore from 2012 through 2015.\model, enables John to formalizes their domain knowledge as abstract \emph{concepts}, e.g., the ``protests'' concept in \autoref{fig:model-design:domain-analytic-knowledge}, and specific \emph{instances} of these concepts, e.g., the ``Baltimore protests'' instance in \autoref{fig:model-design:domain-analytic-knowledge}~\cite{gotz_interactive_2006}. To develop analytic knowledge, analysts infer \emph{relationships} from a given dataset~\cite{pirolli_sensemaking_2005,gotz_interactive_2006,yang_chen_toward_2009,srinivasan_augmenting_2019}, such as by visualizing potential trends or testing correlations through computational models, e.g., calculating a linear regression as shown in \autoref{fig:model-design:domain-analytic-knowledge}. To prepare the data for visualization or modeling, analysts apply \emph{data transformations}~\cite{heer2021arquero,satyanarayan2017vega-lite,yang_chen_toward_2009}, such as deriving new data attributes for further analysis, aggregating the data to calculate summary statistics, or filtering the data to remove irrelevant records as shown in \autoref{fig:model-design:domain-analytic-knowledge}.



\subsection{Domain Knowledge Example}

\model\ enables us to formalize John's domain knowledge as abstract \emph{concepts}, e.g., the ``protests'' and specific \emph{instances} of these concepts, e.g., the ``Baltimore protests.'' We define the concepts ``Crime'' and ``Protest'' (lines 1-8). Then, we define an instance of the ``Protest'' concept based on the Baltimore Protests in 2015. \revised{This instance is recorded directly as the properties of a new domain knowledge node (lines 9-22). Each node represents a specific instance, which} is associated with a core concept and (optional) relevant concepts.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=.8\columnwidth]{figures/domainknowledge.png}
%     \caption{\model\ domain knowledge specification example.
%     }
%     \label{fig:domain-knowledge}
% \end{figure}

\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
const crime = new Concept(
  name: "Crime", // name
  [] // parentConcepts
);
const protest = new Concept(
  "Protest", // name
  [] // parentConcepts
);
const protestsNode = new DomainKnowledgeNode(
    "2015BaltimoreProtests", // name
    protest, // coreConcept, instance property
    { // metadata, instance property
        attributes: [{
            name: "link",
            attributeType: AttributeType.nominal
        }],
        values: {
            "link": "https://en.wikipedia.org/wiki/" +
            "2015_Baltimore_protests"
        }
    }
);
\end{minted}
\end{minipage}
\vspace{1em}

Researchers can link instances together by programming edges between their corresponding nodes which represent different conceptual relationships, such as one node ``causing'' another node, suggesting a directed relationship between the two nodes, or one node being ``related to'' another node, suggesting a general link but no causal direction. To link a source (i.e., parent) node, we call the \texttt{addSource} function on the \texttt{protestsNode} object; similarly, we call \texttt{addTarget} to add a target (i.e., child) domain knowledge node. Related nodes can be linked using the \texttt{addRelated} function.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/example_overview2.pdf}
    \caption{\revised{An overview of how the major components of \model{} connect to form insights, objectives and tasks, demonstrated by the illustrative example in \autoref{sec:protest_example} recreating an analysis scenario where John, a (fictitious) analyst, investigates a crime peak in Baltimore that coincides with protests in the area~\cite{mathisen_insideinsights_2019}. The grey nodes represent the specified \model{} objects from this example. Each node is labeled with its corresponding theoretical component from \autoref{sec:model-design}, shown in italics. The directed edges represent input relationships. For example, the \texttt{protest} object is an input to the \texttt{protestsNode} object.}}
    \label{fig:crimetask-overview}
\end{figure*}

\subsection{Analytic Knowledge Example}
To develop analytic knowledge, analysts infer \emph{relationships} from a given dataset~\cite{pirolli_sensemaking_2005,gotz_interactive_2006,yang_chen_toward_2009,srinivasan_augmenting_2019}, such as by visualizing potential trends or testing correlations through computational models, e.g., calculating a linear regression. To prepare the data for visualization or modeling, analysts apply \emph{data transformations}~\cite{heer2021arquero,satyanarayan2017vega-lite,yang_chen_toward_2009}, such as deriving new data attributes for further analysis, aggregating the data to calculate summary statistics, or filtering the data to remove irrelevant records. We demonstrate the application of these ideas through our continuing example.
To start, we demonstrate how to create \emph{data transformations} by using Arquero to calculate total reported crimes per day and identify peak crime days.

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=.8\columnwidth]{figures/datatransformation.png}
%    \caption{\model\ data transformation example.
%    }
%    \label{fig:datatransformation}
%\end{figure}

\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
// Arquero Data Transformation
const aggTransform = {
    sources: [baltimoreCrime],
    transforms: [
      // group by day
      { op: "groupby", args: ["CrimeDate"] },
      // count crimes per day
      { op: "rollup", args: [{ count: op.count() }] },
      // sort days by count
      { op: "orderby", args: [desc("count")] },
      // return top 3 days with highest counts
      { op: "filter", args: [() => op.rank() <= 2] }
    ]
};
 const getAggTransformResults =
  () => executeDataTransformation(aggTransform);
\end{minted}
\end{minipage}
\vspace{1em}

First, we specify the input datasets, in this case the Baltimore crime dataset (line 3). Then, we list the transforms to execute: group the reported crimes by date (line 6), count total records per day (line 8), sort the dates by count (line 10), and filter for only the top three dates with the highest counts (line 12). Finally, we can execute the transformations on the data using the \texttt{executeDataTransformation} method on line 16.

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=.8\columnwidth]{figures/analyticknowledge.png}
%    \caption{\model\ analytic knowledge specification example.
%    }
%    \label{fig:analytic-knowledge}
%\end{figure}

\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
const crimePeaks = new AnalyticKnowledgeNode(
  "peakCrimes", // node name
  Date.now(), // timestamp
  aggTransform, // data transformation
  null, // data relationship
  getAggTransformResults, // results
  "top 3 days of reported crimes" //  [optional] description
);
\end{minted}
\end{minipage}
\vspace{1em}


Then, we can record how John processed the data to identify peaks in a new analytic knowledge node.
First, we give this unit of analytic knowledge a name (line 2) and when he learned this knowledge (line 3). Then, we connect any relevant data transformations and/or relationships (lines 4-5). In this case, John's findings relate only to the \texttt{aggTransform} object. Optionally, we can add notes about what John learned as a final parameter (line 7).
Similar to domain knowledge nodes, we can link to other analytic knowledge nodes using \texttt{addSource}, \texttt{addTarget}, and \texttt{addRelated}. All node objects in \model\ share this linking property.

\model\ can also record \textit{data relationships} in analytic knowledge nodes, \revised{which can be used to express statistical or mathematical information about a dataset (see \autoref{sec:model-design:data-relationship})}. Consider the following extension of the Baltimore example: suppose John is interested in determining whether location is indicative of crime type, for example, whether different crimes happen indoors versus outdoors, or in an apartment versus a business. We can specify a new model to predict this relationship as follows:


\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
const descRel = new DecisionTreeClassificationRelationshipModel(
  "predictCrimeType", // name
  [ // input attributes to predict with
    {
      name: "Inside/Outside",
      attributeType: AttributeType.nominal
    },
    {
      name: "Premise",
      attributeType: AttributeType.nominal
    }
  ],
  // output attribute to be predicted
  {
    name: "Description",
    attributeType: AttributeType.nominal
  }
);
dt.train(baltimoreCrimes.records);
const prediction = dt.predict(baltimoreCrimes.records[0]);
\end{minted}
\end{minipage}
\vspace{1em}



\revised{Note that since the input and output attributes are categorical, numeric relationships such as linear regression are inappropriate to express this data relationship. Instead, }
we specify a decision tree classifier to predict the relationship (line 1). The input attributes used to train the model are ``Inside/Outside'' and ``Premise'' (lines 3-12). The output attribute being predicted is ``Description'' (lines 14-17), which describes the type of crime reported. \revised{However, using a machine learning relationship is not required, and the model type can easily be swapped in \model{} by choosing a relationship type other than \texttt{DecisionTreeClassificationRelationshipModel}.}

\model\ enables one to not only specify data relationships but also compute them directly on the input data. For example, Line 19 shows how we can train the specified decision tree model on the Baltimore crimes dataset using \model, and Line 20 shows how this model can be used to predict the crime type of specific records. In this way, specified analytic knowledge can be evaluated for statistical rigor by testing the accuracy of the underlying data relationships, supporting prior calls for more precise evaluation of user insights~\cite{zgraggen_investigating_2018}.

\revised{Suppose that \texttt{Inside/Outside} and \texttt{Premise} do not seem to be strong predictors of crime \texttt{Description}. We can record this result using a new AnalyticKnowledgeNode as follows:}

\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
const crimeLoc = new AnalyticKnowledgeNode(
  "crimeLocations", // node name
  Date.now(), // timestamp
  null, // data transformation
  descRel, // data relationship
  null, // results
  "location poor predictor of crime type" //  [optional] description
);
\end{minted}
\end{minipage}
\vspace{1em}

Note that \model\ supports multiple models for capturing multivariate relationships, such as K nearest neighbors, linear regression, and naive Bayes models, as well as univariate relationships (e.g., via kernel density estimation) and other statistical relationships such as outliers (e.g., via isolation forests).

\subsection{Insight Example} The last step in specifying insights is to link domain knowledge with relevant analytic knowledge. Continuing our example, we specify an insight connecting John's domain knowledge about the Baltimore protests (line 3) and analytic knowledge regarding peak crime dates in Baltimore (line 4):

\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
const johnsInsight = new InsightNode(
  "johnsInsight", // name
  [protestsNode], // domain knowledge
  [crimePeaks, crimeLoc], // analytic knowledge
  "Peak Crime = Freddy Grey's Funeral." + // [optional] description
    "location not as relevant."
);
\end{minted}
\end{minipage}
\vspace{1em}

\revised{We can also keep track of John's ``dead ends'' as desired, for example including our \texttt{crimeLoc} analytic knowledge node as shown on line 4.} Similar to the domain and analytic knowledge nodes, insight objects are also nodes, and thus support the linking of source, target, and related insights.


\begin{comment}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/obj-task-insight-crimetask.png}
    \caption{We present an example of our specification language demonstrating the connection between tasks, objectives, and insights. Here, we use an illustrative scenario that follows a fictional crime analyst as he investigate a crime peak in Baltimore that coincides with protests in the area~\cite{mathisen_insideinsights_2019}. \textbf{(b)} demonstrates the programmatic definition of an analytic task as a pairing of an objective, \textbf{(a)}, and an insight, \textbf{(c)}. We specify an insight as a link between domain and analytic knowledge as exemplified by \textbf{(d)} and \textbf{(e)}. Finally, \textbf{(f)} demonstrates how the language enables data transformations. \leilani{out of date. Needs to be updated to match the new \model{} format. Ideally, we should create everything directly in powerpoint rather than snapshots.}}
    \label{fig:crimetask-overview}
\end{figure*}
\end{comment}




%%%%%%%%%%%%%%
% Objective
%%%%%%%%%%%%%%



\subsection{Objective Example}

We demonstrate the use of a wildcard below, denoted with ``*''.
In this case, we have a complete specification for domain knowledge (line 3) but not for analytic knowledge (line 4). This suggests that John wants to explore a range of analyses that may potentially connect data with his existing domain knowledge, which we can frame as an analysis question: \emph{How did the date of Freddy Gray's funeral (April 27, 2015) impact crime in Baltimore?}

\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
const protestsObjective = new InsightNode(
  "protestsObjective", // name
  [protestsNode], // domain knowledge
  "*", // analytic knowledge
  "How did Freddy Gray's funeral impact Baltimore crime?" // [optional] description
);
\end{minted}
\end{minipage}
\vspace{1em}


Now, suppose we stepped backward into John's analysis timeline where he had initially uncovered the crime peak on April 27, 2015, but before he learned about Freddy Gray's funeral. We can reframe the corresponding objective as the following question: \emph{What happened on April 27, 2015 that may have led to more crime?} In this example, we specify analytic knowledge (line 4) and the wildcard appears for domain knowledge (line 3):

\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
const aprilCrimeObjective = new InsightNode(
  "aprilCrimeObjective", // name
  "*", // domainKnowledge
  [crimePeaks], // analyticKnowledge
  "What happened on April 27, 2015 that may have led to more crime?" // [optional] description
);
\end{minted}
\end{minipage}
\vspace{1em}



Note that we can also include wildcards within nested properties, for example within a data relationship or data transform (see supplemental materials for more details).
%other examples of using wildcards (e.g., data transforms) in the supplementary material. \ao{confirm this and maybe specify which section?}
%\leilani{We don't have examples of wildcards in the supplementary material.}

\subsection{Task Example}
\label{sec:protest_example:task}


Using our Baltimore crimes example, we can specify John's analysis task as shown below.
In this case, John has an objective to explore potential relationships between protests and incidence of crime, represented by the \texttt{protestsObjective} object in line 3. In pursuing this objective, he arrives at an insight, represented by the array containing the \texttt{protestsInsight} object in line 4.



\vspace{1em}
\begin{minipage}{.9\linewidth}
\begin{minted}
{javascript}
const protestsTask = new SimpleTaskNode(
  "protestsTask", // name
  protestsObjective, // objective
  [protestsInsight], // insights
);
\end{minted}
\end{minipage}
\vspace{1em}




==> old/related-work.tex <==
\revised{\section{Related Work}}
\label{sec:related-work}

\revised{In this section, we summarize relevant concepts that intersect with visualization task theory and our design of \model{}.}


\subsection{\revised{Theoretical Models in Visualization}}
\label{sec:related-work:languages}

\revised{Theoretical models can help bridge the gap between the high-level human behaviors that researchers observe in the real world and the low-level instructions understood by computers. We briefly summarize the strengths and limitations of different model types observed in visualization theory work.}

\vspace{-2mm}
\revised{\paragraph{Conceptual Models.} Conceptual models are popular theoretical contributions, such as the model of distributed cognition discussed by Liu et al.~\cite{liu2008distributed}, the nested model for visualization design and validation proposed by Munzner~\cite{munzner_nested_2009}, the taxonomy of visualization tasks proposed by Brehmer and Munzner~\cite{brehmer_multi-level_2013}, and the flow chart of visualization construction cycles proposed by Grammel et al.~\cite{grammel2010how}. Conceptual theories are useful for summarizing general purpose principles in visualization, such as guiding how researchers reflect on their approach to designing visualization tools. However, conceptual models are difficult to incorporate into software, and require significant effort from other researchers to interpret and program. For example, Gathani et al. attempted to map seven existing taxonomic models to deterministic labeling programs for analyzing user interaction logs, and found that many existing taxonomies lack sufficient specificity to generate meaningful labels for recorded interactions~\cite{gathani2022grammar}.}

\vspace{-2mm}
\revised{\paragraph{Mathematical Models.} An alternative approach is to provide \emph{mathematical} formulations to approximate observed behavioral patterns, such as mathematical equations for modeling graphical perception~\cite{harrison2014ranking,kindlmann_algebraic_2014}, visualization properties~\cite{demiralp_visual_2014}, or user intent~\cite{bertin1983semiology}. Unlike conceptual models, mathematical models can easily be programmed into visualization tools. However, mathematical equations often have a narrow scope~\cite{demiralp_visual_2014}, and as a result cannot account for nuance and complexity in human behavior. For example, although the Weber-Fechner equation can capture some facets of graphical perception~\cite{harrison2014ranking}, a comprehensive model of graphical perception would likely outstrip its expressive capabilities~\cite{kay2016beyond}.}

\vspace{-2mm}
\revised{\paragraph{Programmatic Models.} A more flexible alternative is to propose \emph{programmatic} models for capturing visual analysis behavior, which can strike a balance between the generalizability of conceptual models and the precision of mathematical models.  The strength of programmatic models is demonstrated through their use in modeling the visualization design space~\cite{zeng2022evaluation}. For example, automated visualization design tools have a long history of leveraging programmatic models of user intent, including Mackinlay's work on the APT system~\cite{mackinlay1986automating}, and continuing with more recent work, such as Stolte et al.'s a table algebra
to power Polaris/Tableau~\cite{stolte2002polaris}, Wongsuphasawat et al.'s use of two languages (CompassQL~\cite{wongsuphasawat2016towards} and Vega-Lite~\cite{satyanarayan2017vegalite}) to develop Voyager~\cite{wongsuphasawat_voyager_2017}, Mortz et al.'s use of answer set programming to power Draco~\cite{moritz2018formalizing}, and the community's panoply of successful visualization specification languages based on the Grammar of Graphics~\cite{wilkinson2012grammar}, including ggplot2 (based on Wickham's layered grammar of graphics~\cite{wickham2010layered}) and Vega-Lite~\cite{satyanarayan2017vegalite}. However, programmatic formulations are not limited to visualization specification. For example, regular expressions can be used to enable programmatic generation of new interaction taxonomies~\cite{gathani2022grammar}. Furthermore, domain-specific languages such as SQL are frequently used to express user analysis intent~\cite{mcnutt2022grammar}.}

\revised{That being said, programmatic models are not a panacea. For example, they are often verbose and complex, whereas mathematical and conceptual models are generally concise. Furthermore, programmatic models can be difficult to understand due to their complexity. For example, SQL is notoriously difficult to debug~\cite{gathani2020debugging}, and even visualization specification languages can be unintuitive at times~\cite{satyanarayan2020critical}. Even with their limitations, we observe many successful programmatic models in the literature, which guided our decision to develop \model{}. For example, although many conceptual models of insight have been proposed, we have yet to see languages for specifying \emph{insights} and their \emph{relationships} to users' objectives and tasks~\cite{kandogan2018towards}. We address this gap through \model{}.}

%In this paper, we focus on the construction of theoretical models for creating and drawing insights from visualizations, which can then be used by software to interpret and reason about user interactions.

\subsection{\revised{Visualization Provenance}}
\label{sec:related-work:provenance}

\revised{Here, we briefly summarize key takeaways on visualization provenance; we defer to established surveys in data, workflow and analytic provenance for in-depth details~\cite{xu_survey_2020,ragan2016characterizing,davidson2008provenance,cheney2009provenance,gathani2022grammar,battle_characterizing_2019}.
A key feature of many modern visualization tools is intelligent and responsive design, where the tool is designed to infer and even anticipate a user's analysis needs~\cite{xu_survey_2020,battle2021structured,zeng2022evaluation}. Visualization recommendation tools~\cite{zeng2022evaluation}, big data exploration tools~\cite{battle2021structured}, and bias mitigating tools~\cite{wall2017warning,wall2022left} are prominent examples.}

\revised{Interpreting and responding to user needs requires an understanding of the user's analysis intent~\cite{rind_task_2016,battle_characterizing_2019,brehmer_multi-level_2013,lam_bridging_2018}.
As a result, a large body of visual analytics research is devoted to \emph{provenance}, or collecting and analyzing a user's interactions with and queries within visual analysis tools~\cite{xu_survey_2020,ragan2016characterizing}. For example, interaction and data provenance can be used to infer user intent (e.g., \cite{ottley_follow_2019,battle2016dynamic,yan2021tessera,gathani2022grammar}) as well as to design features to accommodate various visual analysis tasks (e.g., \cite{battle_characterizing_2019,monadjemi_competing_2020,pandey2022medley}). However, user tasks are generally recorded \emph{indirectly} through analysis of interaction logs~\cite{xu_survey_2020}, contributing to inconsistencies in how tasks are studied in visualization~\cite{rind_task_2016}. Furthermore, we observe no consistent frameworks for recording insights within visualization tools, whereas we \emph{do} see them for interaction logging (e.g., \cite{cutler2020trrack}). We propose a theory-driven approach to recording the \emph{intents} behind and \emph{results} of analysis activity, with the goal of elevating the importance of insights, objectives and tasks alongside interaction logs within provenance-based research.}

\subsection{\revised{Knowledge Graphs}}
\label{sec:related-work:knowledge-graphs}

\revised{Here, we provide a brief introduction to the concept of knowledge graphs, and defer to established surveys for more details~\cite{hogan2021knowledge,ji2021survey}. A knowledge graph is ``\emph{a graph of data intended to accumulate and convey knowledge of the real world, whose nodes represent entities of interest and whose edges represent potentially different relations between these entities}''~\cite{hogan2021knowledge}. A prominent example is Wikidata~\cite{vrandevcic2014wikidata}, a popular knowledge graph backing Wikipedia and other relevant open source projects. A knowledge graph with formal semantics for automated reasoning is also often referred to as a \emph{knowledge base}~\cite{ji2021survey}. In this paper, we specify knowledge graphs with formal semantics among and between graph nodes, so we use the terms knowledge graph and knowledge base interchangeably.}

\revised{Entities, the nodes of a knowledge graph, can take a variety of forms, including physical objects such as cities and people~\cite{hogan2021knowledge}, as well as digital objects such as web pages and structured datasets~\cite{bizer2009linked}.
The edges of a knowledge graph are used to record relationships between entities~\cite{hogan2021knowledge,ji2021survey}, such as which cities are located within certain countries or hyperlinks between web pages (e.g., Wikipedia pages) and their backing data (e.g., Wikidata).}

\revised{Visualization research in insight discovery also discusses how insights drawn from visualizations can extend a user's knowledge base~\cite{gotz_interactive_2006,chang_defining_2009}, which can be represented as establishing new nodes and links within a knowledge graph~\cite{kandogan2018towards}. Specifically, insight is often described as links forged between analysis results and user knowledge~\cite{gotz_interactive_2006,pousman_casual_2007,shrinivasan_supporting_2008,smuc_score_2009,kandogan2018towards}, and even defined as a knowledge building activity in general~\cite{chang_defining_2009}.
%As an example, Gotz et al. describe how government intelligence analysts may link specific persons of interest with recent events that reveal threats to local or national security~\cite{gotz_interactive_2006}. Gotz et al. also define separate entities to capture the knowledge analysts gain from data visualizations (analytic knowledge), which can also be linked with these persons of interest and relevant events.
Through \model{}, we extend prior work to enable precise specification of insights, objectives, and tasks, which can be linked together to formalize our understanding of how a user's knowledge base is augmented through visual data analysis. We review how the visualization literature defines insights, objectives, tasks, and knowledge building in \autoref{sec:background}.}

